End-to-End Deep Learning for Structural Brain Imaging: A Unified Framework

Brain imaging analysis is fundamental in neuroscience, providing valuable insights into brain structure and function. Traditional workflows follow a sequential pipeline-brain extraction, registration, segmentation, parcellation, network generation, and classification-treating each step as an independent task. These methods rely heavily on task-specific training data and expert intervention to correct intermediate errors, making them particularly burdensome for high-dimensional neuroimaging data, where annotations and quality control are costly and time-consuming. We introduce UniBrain, a unified end-to-end framework that integrates all processing steps into a single optimization process, allowing tasks to interact and refine each other. Unlike traditional approaches that require extensive task-specific annotations, UniBrain operates with minimal supervision, leveraging only low-cost labels (i.e., classification and extraction) and a single labeled atlas. By jointly optimizing extraction, registration, segmentation, parcellation, network generation, and classification, UniBrain enhances both accuracy and computational efficiency while significantly reducing annotation effort. Experimental results demonstrate its superiority over existing methods across multiple tasks, offering a more scalable and reliable solution for neuroimaging analysis. Our code and data can be found at https://github.com/Anonymous7852/UniBrain

==> fig_family.tex <==



\begin{table}[ht]
\vspace{-0pt}
\caption{Related works in brain imaging analysis. The gray boxes represent the scope of tasks supported by the methods in the boxes.}
\vspace{-0pt}
\centering
\resizebox{0.9\linewidth}{!}{%
% \begin{tabular}{|c|c|c|cccc|} 
\begin{tabular}{|c|c|c|cccc|} 

\hline

\multicolumn{1}{|c|}{} & 
\multicolumn{6}{c|}{\rule{0pt}{15pt}\LARGE{\textbf{Tasks}}\rule[-5pt]{0pt}{0pt}}

\\
\hline
\includegraphics[width=1.2cm]{fig/fig_family/raw.png}   & \includegraphics[width=1.2cm]{fig/fig_family/ext.png}               & \includegraphics[width=1.2cm]{fig/fig_family/reg.png}               & \multicolumn{1}{c|}{\includegraphics[width=1.2cm]{fig/fig_family/seg.png}}               & \multicolumn{1}{c|}{\includegraphics[width=1.2cm]{fig/fig_family/parc.png}}              & \multicolumn{1}{c|}{\includegraphics[width=1.2cm]{fig/fig_family/ng_v2.png}}              & \includegraphics[width=1.2cm]{fig/fig_family/cls_v3.pdf}               \\ 
\hline
\multirow{2}{*}{Raw}                       & \multirow{2}{*}{\textbf{Extraction}}                             & \multirow{2}{*}{\textbf{Registration}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Segmentation}}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Parcellation}}}                         & \multicolumn{1}{c|}{\textbf{Network}}                   & \multirow{2}{*}{\textbf{Classification}}                        \\ 

\multicolumn{1}{|c|}{} &
\multicolumn{1}{c|}{} &
\multicolumn{1}{c|}{} &
\multicolumn{1}{c|}{} &
\multicolumn{1}{c|}{} &
\multicolumn{1}{c|}{\textbf{Generation}} &
\multicolumn{1}{c|}{} \\

\hline
& {\cellcolor[rgb]{0.753,0.753,0.753}}\cite{smith2002fast,cox1996afni,shattuck2002brainsuite,hoopes2022synthstrip} & \multicolumn{1}{|c}{}                  &                                                            &                                                           &                                                           &                                       \\ 
\hhline{|~--~~~~|}
                          &                                       & {\cellcolor[rgb]{0.753,0.753,0.753}}\cite{jenkinson2001global,balakrishnan2018unsupervised,zhao2019recursive,su2022abn} &                                                            &                                                           &                                                           &                                       \\ 
\hhline{|~~--~~~|}
                          & \multicolumn{1}{c}{}                  &                                       & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\cite{akkus2017deep, kamnitsas2017efficient,chen2018voxresnet,jaderberg2015spatial}} &                                                           &                                                           &                                       \\ 
\hhline{|~~~--~~|}
                          & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  & \multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\cite{thyreau2020learning,lim2022deepparcellation,jaderberg2015spatial}} &                                                           &                                       \\ 
\hhline{|~~~~--~|}
                      \multirow{1}{*}{Related}    & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  &                                                            & \multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}\cite{liang2012effects,zhou2020toolbox,sporns2013structure,vskoch2022human}}} &                                       \\ 
\hhline{|~~~~~--|}
                       \multirow{1}{*}{Works}   & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  &                                                            &                                                           & \multicolumn{1}{c|}{}                                     & {\cellcolor[rgb]{0.753,0.753,0.753}\cite{li2021braingnn,kawahara2017brainnetcnn,li2023interpretable, kan2022brain}}  \\ 
\hhline{|~--~~~-|}
                          & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\cite{su2022ernet}}                    &                                                            &                                                           &                                                           &                                       \\ 
\hhline{|~---~~~|}
                          &                                       & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\cite{qiu2021u, xu2019deepatlas,he2020deep}}                                         &                                                           &                                                           &                                       \\ 
\hhline{|~---~~~|}
                          & \multicolumn{3}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\cite{su2023one}}                                                                                 & \multicolumn{1}{l}{}                                      & \multicolumn{1}{l}{}                                      & \multicolumn{1}{l|}{}                 \\ 
\hhline{|~---~--|}
                          & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                                       & \multicolumn{1}{l|}{}                                     & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\cite{kan2022fbnetgen,mahmood2021deep,yu2023deep}}                                       \\ 
\hhline{|~------|}
                          & \multicolumn{6}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\textbf{Unified model for end-to-end brain network analysis (ours)}}                                                                                                                                                                                                                                                \\
\hline
\end{tabular}
}
\label{tab: family}
\vspace{-0pt}
\end{table}



==> fig_formulation.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/function_v4.png}
  \vspace{-12pt}
  \caption{A demonstration of extraction, registration and segmentation functions.}
  \label{fig:formulation}
  \vspace{-15pt}
\end{figure}

==> fig_main_res_v2.tex <==

\definecolor{mypgreen}{RGB}{142, 179, 142}
\definecolor{mypred}{RGB}{181, 83, 53}
\definecolor{myppurple}{RGB}{175, 145, 185}
\definecolor{mypyellow}{RGB}{206,226,46}



\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{fig/main_result.pdf}
  \vspace{-6pt}
  \caption{
  %Visual comparisons for brain extraction, registration, segmentation, and parcellation tasks. We show 3D visualizations and middle slices in sagittal, axial, and coronal planes. On the left, source and target (template) images are displayed with their ground truth labels.
  %The results and predicted labels for each method in extraction, registration, segmentation and parcellation are illustrated for performance assessment. 
  %Successful extraction, segmentation and parcellation imply a high overlap between predicted and ground truth masks. For registration, the higher similarity between the registered and template brains indicates better performance.
  Visual comparisons for brain extraction, registration, segmentation, and parcellation tasks include 3D visualizations and middle slices in sagittal, axial, and coronal planes. Source and target images with ground truth labels are shown on the left. Predicted masks and results for each method are displayed for assessment. High overlap between predicted and ground truth masks indicates successful extraction, segmentation, and parcellation. For registration, higher similarity between the registered and template brains indicates better performance.
  }
  \label{fig:main result}
  \vspace{-6pt}
\end{figure*}

==> fig_network1.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/method.pdf}
  \caption{Model architecture of the proposed SkipSNN.}
  \label{fig:model}
  \vspace{-10pt}
\end{figure*}



==> fig_network2.tex <==



\definecolor{myext}{RGB}{181, 181, 181}
\definecolor{myreg}{RGB}{251, 153, 140}
\definecolor{mysegparc}{RGB}{218, 175, 244}
\definecolor{mybn}{RGB}{249, 203, 156}
\definecolor{mypre}{RGB}{255, 127, 80}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{fig/method_v16.png}
    \vspace{-5pt}
  \caption{Overview of the UniBrain. \textbf{\textcolor{myext}{Extraction (Ext)}} module removes non-brain tissue of the raw source image~$\mathbf{S}$, producing the extracted brain image~$\mathbf{E}$. \textbf{\textcolor{myreg}{Registration (Reg)}} module aligns extracted brain~$\mathbf{E}$ with the target image~$\mathbf{T}$ through affine transformation~$\mathbf{A}$, resulting in the warped image~$\mathbf{W}$. \textbf{\textcolor{mysegparc}{Segmentation \& parcellation (Seg \& Parc)}} module takes the source image~$\mathbf{S}$, target segmentation mask~$\mathbf{B}$, target parcellation mask~$\mathbf{P}$, and inversed affine transformation~$\mathbf{A^{-1}}$ to generate the segmentation mask~$\mathbf{R}$ and the parcellation mask~$\mathbf{U}$. \textbf{\textcolor{mybn}{Brain~network~(BN)}} module uses the source image~$\mathbf{S}$ and the parcellation mask~$\mathbf{U}$ to construct brain network~$G$.
  %by learning ROI feature~$\mathbf{H}$ and connectivity matrix~$\mathbf{C}$. 
  \textbf{\textcolor{mypre}{Classification (CLS)}} module then uses the ROI feature~$\mathbf{H}$ and connectivity matrix~$\mathbf{C}$ contained in $G$ to produce the prediction~$\hat{y}$. 
  %The final outputs include the extracted brain image~$\mathbf{E}$, the target-aligned warped image~$\mathbf{W}$, the source image's brain tissue segmentation mask~$\mathbf{R}$, the source image's brain ROI parcellation mask~$\mathbf{U}$, the brain network connectivity matrix~$\mathbf{C}$ and the prediction $\hat{y}$.
  }
  \label{fig:network}
  \vspace{-5pt}
\end{figure*}


==> lambda.tex <==


\begin{figure}[t]
    \subfigure[Accuracy on N-MNIST]{
        \includegraphics[width=0.22\textwidth]{fig/nmnist.pdf}
    }
    \subfigure[Accuracy on DVS-Gesture]{
        \includegraphics[width=0.22\textwidth]{fig/dvs.pdf}
    }
    \vspace{-5pt}
    \caption{Observing the performance of different models with different percentage of updated time-steps.}
    \label{fig:lambda}
    \vspace{-10pt}
\end{figure}

==> sec_1_intro_v3.tex <==
%\vspace{-6pt}
\section{Introduction}
\label{sec:intro}
\input{fig_problem}
\textbf{Background.} 
Brain imaging analysis, particularly in using structural neuroimaging, has become a widely adopted paradigm in neuroscience, supporting applications such as anatomical studies~\cite{zhang2024brant,yin2023multi,papalexakis2014good},
multi-modality fusion~\cite{cai2018deep}, brain signal reconstruction~\cite{luo2024brain,scotti2024reconstructing}, diagnostic assistance~\cite{sun2009mining,huang2011brain}, and clinical interpretation~\cite{li2021braingnn}.
This analysis typically involves multiple processing tasks, including brain extraction (\emph{a.k.a.} skull stripping), registration, segmentation, parcellation, network generation, and classification. 
Brain extraction removes non-brain tissues (\eg skull and dura) from an imaging scan, while registration aligns the extracted brain with a standard template. Segmentation focuses on tissue classification, dividing the brain into broad tissue types such as gray matter, white matter, and cerebrospinal fluid (CSF). Parcellation further subdivides the brain into smaller, anatomically distinct regions, such as the frontal, temporal and occipital lobes. Network generation constructs a brain network based on the connectivity among these parcellated regions, and classification is used for clinical prediction. These tasks serve as fundamental steps in many structural neuroimaging studies.

% labels brain tissue types (\eg gray matter, white matter) in the raw imaging scan, and parcellation further subdivides the brain into smaller, more specific regions (\eg frontal lobe, temporal lobe) based on functional, structural, or connectivity patterns; network generation constructs a brain network based on the connectivity among parcellated regions; finally, the classification focuses making clinical predictions. These tasks are preliminary but essential in many neuroimaging studies. 
For example, in brain anatomical analysis, extraction and registration assist in eliminating interference from non-cerebral tissues, imaging modalities, and differing viewpoints. Segmentation and parcellation enable the measurement and analysis of anatomical variations observed in specific brain tissues and regions.
Network generation and classification facilitate graph theory for interpretation and prediction. 
In disease diagnosis, the brain must first be extracted from raw imaging scans and aligned with a standard template (\eg MNI152) to eliminate inter-individual variations. Next, intra-individual structural abnormalities (\eg brain atrophy) across different pathological stages should be monitored through anatomical analysis (\eg identify the corresponding brain tissue and measure volumetric changes). At the group level, functional impairments (\eg frontal lobe decline) can be detected and interpreted by analyzing regional connectivity through brain network analysis. These comprehensive assessments play a crucial role in assisting physicians in making accurate and reliable diagnoses.

% \noindent\textbf{Problem Definition.} 

This paper aims to revolutionize current methodologies by establishing an integrated, end-to-end deep learning architecture, \textbf{UniBrain}, that streamlines and optimizes the entire brain image processing pipeline. 

In this paper, we study the problem of end-to-end learning for brain imaging tasks, as shown in Figure~\ref{fig:intro}. 
The objective is to explore how tasks like brain extraction, registration, segmentation, parcellation, network generation, and classification interrelate, aiming to mutually boost their efficacy with minimal labeled data. Specifically, we utilize low-cost labels (\ie extraction mask, classification label) and only one labeled template (\emph{a.k.a.} atlas) to perform all tasks simultaneously. Notably, our goal is to avoid using any of the instance-level ground-truth labels of registration, segmentation, parcellation, and network connectivity in model training.

\noindent\textbf{Related Works.} 
In the literature, related tasks in brain imaging analysis have been extensively studied. Conventional methods primarily focus on designing methods for brain extraction~\cite{kleesiek2016deep,lucena2019convolutional}, registration~\cite{sokooti2017nonrigid, su2022abn}, segmentation~\cite{akkus2017deep, kamnitsas2017efficient, chen2018voxresnet}, parcellation~\cite{thyreau2020learning,lim2022deepparcellation}, network generation~\cite{zhou2020toolbox,vskoch2022human} and classification~\cite{li2021braingnn,kawahara2017brainnetcnn, kan2022brain} separately under supervised settings. However, in brain imaging studies, the collection of voxel-level annotations, transformations between images, and task-specific brain networks often prove to be expensive, as it demands extensive expertise, effort, and time to produce accurate labels, especially for high-dimensional neuroimaging data, \eg 3D MRI. To reduce this high demand for annotations, recent works have utilized automatic extraction tools~\cite{smith2002fast,cox1996afni,shattuck2002brainsuite, segonne2004hybrid}, unsupervised registration models~\cite{balakrishnan2018unsupervised,su2022abn}, inverse warping~\cite{jaderberg2015spatial}, and correlation-based metrics~\cite{liang2012effects} for performing extraction, registration, segmentation, parcellation and network generation. Nevertheless, these pipeline-based approaches frequently rely on manual quality control to correct intermediate results before performing subsequent tasks. Conducting such visual inspections is not only time-consuming and labor-intensive but also suffers from intra- and inter-rater variability, thereby impeding the overall efficiency and performance. More recently, joint extraction-registration~\cite{su2022ernet}, joint registration-segmentation~\cite{xu2019deepatlas}, joint extraction-registration-segmentation~\cite{su2023one}, and joint network generation-classification~\cite{kan2022fbnetgen} have been developed for collective learning. However, partial joint learning overlooks the potential interrelationships among all tasks, which can adversely affect overall performance. 
%Related works are demonstrated in Table~\ref{tab: family}.

%\noindent\textbf{Challenges.} Three main challenges arise in the problem of end-to-end learning for brain imaging tasks.

%Despite its value and significance, the problem of end-to-end brain image analysis has not been studied before and is very challenging due to its unique characteristics listed below:

%\textbullet  \  
%\textit{Limited labeled information:} Conventional learning-based methods typically require a substantial collection of ground-truth labels for these tasks. However, acquiring detailed voxel-level labels (\eg tissue type, region location) and transformation labels in high-dimensional neuroimaging data is notably expensive and time-consuming. We minimize reliance on extensive labeling, using only the necessary label (\ie classification label) and a relatively low-cost label (\ie brain extraction masks). Although we provide a template image with its segmentation and parcellation masks (in template image space), the segmentation and parcellation masks (in raw image space) for the raw image are not available. Furthermore, the ground-truth brain network connectivity is also not provided.

%\textbullet  \  
%\textit{Dependencies among all tasks:} Conventional research often treats brain extraction, registration, segmentation, parcellation, network generation, and classification tasks separately. However, these tasks exhibit significant interdependencies: 1) effective extraction (\ie successful removal of non-brain tissue) allows the brain to precisely align to template image, thereby enhancing registration accuracy; 2) precise registration can accurately guide segmentation and parcellation through inverse transformation (\ie inversely warping template masks to the raw image space); 3) accurate parcellation contributes to consistent region divisions across subjects, crucial for generating robust brain networks; 4) networks that precisely capture brain connectivity can substantially improve classification and diagnosis outcomes. Therefore, a holistic approach is essential to manage these interdependencies effectively in an end-to-end framework.

%\textbullet  \  
%\textit{Heterogeneous inputs and outputs across tasks:} Developing a unified model for brain imaging analysis is markedly challenging since all tasks have incredibly diverse input and output representation. For example, extraction results in a binary mask that outlines the brain, while registration yields a transformation matrix for image coordinate mapping. Segmentation and parcellation generate multi-class masks to delineate brain tissues and regions. Network generation produces an adjacency matrix to capture brain region connectivity, and classification outputs categorical labels.
%This heterogeneity makes it very challenging to architect a single end-to-end model for all these tasks.

\noindent\textbf{Proposed Method.} To achieve the goal, we introduce a unified framework, UniBrain, the first model for end-to-end learning of brain imaging analysis tasks. UniBrain comprises a group of modules for extraction, registration, segmentation, parcellation, network generation, and classification. The extraction module removes non-brain tissue from the raw image, yielding an extracted image. The registration module aligns the extracted image with a template. 
The segmentation and parcellation modules generate the segmentation and parcellation masks on the raw image.
Concurrently, the network generation module learns representations of brain regions and constructs a brain network. 
Finally, the classification module makes the final predictions.
By integrating these modules in an end-to-end fashion, UniBrain enables mutual boosting across tasks, achieving joint optimization with limited labeled data.
Extensive experiments on multiple public brain MRI datasets show that our method significantly surpasses existing state-of-the-art approaches in all six tasks.


==> sec_2_problem_def3.tex <==
\section{PRELIMINARIES} 


%In this section, we first introduce the relevant concepts and notations. We then formulate the problem of end-to-end learning for brain imaging tasks. Notations are detailed in Appendix~\ref{section: appendix Details of and Definitions Notations} and Table~\ref{tab: Notation}.

%\subsection{Notations and Definitions}
\noindent \textbf{Definition 1 (Training data).}
Given a training dataset $\mathcal{D} = \{(\mathbf{S}_i,\mathbf{M}_i,y_i)\}_{i=1}^{Z}$, along with a template $(\mathbf{T}, \mathbf{B},\mathbf{P})$. The dataset contains $Z$ source images $\mathbf{S}_{i} \in \mathbb{R}^{W \times H \times D}$ (\eg raw MRI), each paired with a brain extraction mask $\mathbf{M}_i \in \{0,1\}^{W \times H \times D}$ and a classification label $y_i \in \mathcal{Y}$. 
The template contains a target image $\mathbf{T} \in \mathbb{R}^{W \times H \times D}$, with its segmentation mask $\mathbf{B} \in \{0, 1\}^{C \times W \times H \times D}$ and parcellation mask $\mathbf{P} \in \{0, 1\}^{K \times W \times H \times D}$. Here, $W$, $H$, and $D$ denote the width, height and depth dimensions of the 3D images, $C$ denotes the number of segmentation labels (\ie the number of brain tissue types), $K$ denotes the number of brain regions (\ie the number of ROIs). $\mathcal{Y}$ is the classification label space (\eg $\{0, 1\}$ for binary classification). Next, we omit the subscript $i$ of $\mathbf{S}_i$, $\mathbf{M}_i$ and $y_i$ for simplicity.

\noindent \textbf{Definition 2 (Outputs of each task).} 1) \textit{The extraction task} outputs a binary extraction mask $\hat{\mathbf{M}}\in \{0,1\}^{W \times H \times D}$, representing cerebral tissues in source image $\mathbf{S}$ with a value of 1 and non-cerebral tissues with 0. The extracted image $\mathbf{E} = \mathbf{S} \circ \hat{\mathbf{M}}$ is obtained by applying $\hat{\mathbf{M}}$ on $\mathbf{S}$ via an element-wise product $\circ$. 2) \textit{The registration task} outputs a 3D affine transformation matrix $\mathbf{A} \in \mathbb{R}^{4 \times 4}$,
%with 12 degrees of freedom (\ie 3 for rotation, 3 for translation, 3 for scale, and 3 for shear),
indicating the coordinate correspondence between the extracted image $\mathbf{E}$ and the target image $\mathbf{T}$. The warped image (\ie registered image) $\mathbf{W} = \mathcal{T}\left(\mathbf{E},\mathbf{A}\right)$ results from applying the affine transformation on the extracted image $\mathbf{E}$, where $\mathcal{T}(\cdot, \cdot)$ is the affine transformation operator. 3) \textit{The segmentation task} outputs a multi-class segmentation mask $\mathbf{R} \in \{0,1\}^{C \times W \times H \times D}$, categorizing tissue types within the source image $\mathbf{S}$. 
4) \textit{The parcellation task} outputs a multi-class parcellation mask $\mathbf{U} \in \{0,1\}^{K \times W \times H \times D}$, subdividing various regions (ROIs) within the source image $\mathbf{S}$. The parcellated image $\mathbf{F} = \mathbf{S} \circ \mathbf{U}$ is obtained by performing element-wise product $\circ$ between $\mathbf{S}$ and $\mathbf{U}$.
5) \textit{The network generation task} outputs an adjacency matrix $\mathbf{C} \in \mathbb{R}^{K \times K}$ and a 
node feature (\ie ROI feature) matrix  $\mathbf{H} \in \mathbb{R}^{K \times N}$, capturing the brain network connectivity in the source image $\mathbf{S}$ across $K$ ROIs. $N$ is the node feature vector length. 6) \textit{The classification task} outputs a categorical label $\hat{y} \in \mathcal{Y}$, indicating the predictive category.

\noindent \textbf{Problem Formulation.}
Given the limited labeled data and heterogeneous inputs and outputs across tasks, we aim to minimize the need for extensive task-specific labels and enable efficient knowledge transfer across different tasks. Formulating the end-to-end brain imaging analysis as a joint learning problem, we allow interconnected and collective task optimization. Specifically, we designed multiple learnable functions to bridge tasks, while loss terms are jointly optimized by leveraging the limited labeled information. %Without loss of generality, we assume that the transformation in the registration task is affine-based. However, this work can be easily extended to other types of registration, \eg nonlinear/deformable registration.

Formally, our learnable functions are expressed as: the extraction function $f_{\theta}: \mathbb{R}^{W \times H \times D} \rightarrow \mathbb{R}^{W \times H \times D} ; \mathbf{S} \mapsto \hat{\mathbf{M}}$, the registration function $g_{\phi}: \mathbb{R}^{W \times H \times D}\times \mathbb{R}^{W \times H \times D} \rightarrow \mathbb{R}^{4 \times 4} ; (\mathbf{E},\mathbf{T}) \mapsto \mathbf{A}$, the segmentation function $h_{\psi}: \mathbb{R}^{W \times H \times D} \rightarrow \mathbb{R}^{C \times W \times H \times D} ; \mathbf{S} \mapsto \mathbf{R} $, the brain network generation function $n_{\xi}: \mathbb{R}^{K \times W \times H \times D} \rightarrow \mathbb{R}^{K \times N} ; \mathbf{F} \mapsto \mathbf{H} $ and the classification function $c_{\eta}: (\mathbb{R}^{K \times K}, \mathbb{R}^{K \times N}) \rightarrow \mathcal{Y} ; (\mathbf{C},\mathbf{H}) \mapsto \hat{y}$. 
1) \textit{The extraction function} $f_{\theta}(\cdot)$ takes the source
image $\mathbf{S}$ as input to predict the extraction mask $\hat{\mathbf{M}} = f_{\theta}(\mathbf{S})$. 
2) \textit{The registration function} $g_{\phi}(\cdot, \cdot)$ takes the extracted brain image $\mathbf{E} = \mathbf{S} \circ \hat{\mathbf{M}}$ and the target image $\mathbf{T}$ to predict the affine transformation $\mathbf{A} = g_{\phi}(\mathbf{E},\mathbf{T})$, and thereby generating the warped image $\mathbf{W} = \mathcal{T}(\mathbf{E},\mathbf{A})$. Then, the warped segmentation mask $\mathbf{V} = \mathcal{T}(\mathbf{B},\mathbf{A}^{-1})$ 
and parcellation mask $\mathbf{U} = \mathcal{T}(\mathbf{P},\mathbf{A}^{-1})$ are obtained by applying the inverse affine transform $\mathbf{A}^{-1}$ to target segmentation mask $\mathbf{B}$ and parcellation mask $\mathbf{P}$. 
3) \textit{The segmentation function} $h_{\psi}(\cdot)$ predicts source segmentation mask $\mathbf{R} = h_{\psi}(\mathbf{S})$ from the source image $\mathbf{S}$. 
4) \textit{The brain network generation function} $n_{\xi}(\cdot)$ processes parcellated image $\mathbf{F}=\mathbf{S} \circ \mathbf{U}$ to learn the node feature $\mathbf{H} = n_{\xi}(\mathbf{F})$. 
5) \textit{The classification function} $c_{\eta}(\cdot,\cdot)$ takes a learnable adjacency matrix $\mathbf{C} = \mathbf{H} \mathbf{H^\top}$, and node feature $\mathbf{H}$ to make the final prediction $\hat{y}=c_{\eta}(\mathbf{C},\mathbf{H})$.
The optimal parameter set $\mathcal{P^*} = \{\theta^*, \phi^*, \psi^*, \xi^*, \eta^*\}$ can be found by solving the following optimization problem:
\begin{equation}
\label{eq:optimization}
\begin{aligned}
\mathcal{P^*} = \underset{\mathcal{P}}{\arg \min} \sum_{(\mathbf{S}, \mathbf{M}, y)\in \mathcal{D}} \Big[ \mathcal{L}_{cls}\big(\hat{y}, y\big)  & + \alpha \mathcal{L}_{ext}\big(\hat{\mathbf{M}}, \mathbf{M}\big) \\   + \beta  \mathcal{L}_{sim}\big(\mathbf{W}, \mathbf{T}\big)   & + \gamma \mathcal{L}_{seg}\big({\mathbf{R}}, \mathbf{V}\big)\Big],
\end{aligned}
\end{equation}
where the image pair $(\mathbf{S},\mathbf{M},y)$ is sampled from the training dataset $\mathcal{D}$. $\mathcal{L}_{cls}(\cdot, \cdot)$ is classification loss term, $\mathcal{L}_{ext}(\cdot, \cdot)$ is extraction loss term, $\mathcal{L}_{sim}(\cdot, \cdot)$ is image dissimilarity loss term (\eg mean square error), and $\mathcal{L}_{seg}(\cdot, \cdot)$ is segmentation loss term. 
These four criteria leverage the limited labeled information, and guide a joint optimization of extraction, registration, segmentation, parcellation, network generation, and classification, enabling effective interaction and feedback among these tasks.


%To our knowledge, this work is the first endeavor to find an optimal solution for the end-to-end brain imaging analysis problem. Our method unifies all tasks and significantly reduces the need for extensive annotations in brain imaging by utilizing minimal labeled data (\ie extraction mask, classification label, and one labeled template), as opposed to other fully supervised~\cite{sokooti2017nonrigid, dai2020dual,akkus2017deep, kamnitsas2017efficient,chen2018voxresnet,thyreau2020learning,lim2022deepparcellation,zhao2020supervised,zhao2015supervised} and pipeline-based~\cite{smith2002fast,cox1996afni,shattuck2002brainsuite,segonne2004hybrid,balakrishnan2018unsupervised,zhao2019recursive,su2022abn} methods.



==> sec_5_related_work.tex <==
\section{Related Work}
In spike train classification, methods for training SNNs can be divided into two categories: ``Indirect" learning and ``Direct" learning. 
Indirect learning mainly focuses on ANN-to-SNN conversion \cite{diehl2015fast,cao2015spiking,hu2018spiking, midya2019artificial}.
These methods are indirect in that a regular non-spiking Artificial Neural Network (ANN), such as a multi-layer perceptron, is initially used during the training phase. 
At inference-time, the trained model is then converted to an SNN. However, such indirect training doesn't align well with how an SNN operates. For example, in ANNs, it does not matter if activations are negative, while firing rates in SNNs are always positive. As for Direct learning, many methods have recently been proposed \cite{shrestha2018slayer, wu2019direct, yin2021energy}. These approaches train SNNs directly using back-propagation in both the spatial and temporal domains. \cite{shrestha2018slayer,wu2019direct} have achieved state-of-the-art accuracy on the MNIST and N-MNIST datasets. 
\cite{yin2021energy} trains SNNs with a spatial sparsification technique that allows SNNs to perform inference with lower computational cost. While these methods perform better than the indirect methods on many neuromorphic datasets, they are still not suitable for efficient classification of real-world spike trains, especially in terms of temporal-noise problem. 

Although there is no model for dealing with our defined problem for SNNs, some methods have been proposed for dealing with similar problems for RNNs \cite{lalapura2021recurrent, lei2021attention, morais2021learning, zheng2021accurate, hartvigsen2020learning, jernite2016variable, campos2017skip, shen2018ordered}. 
For example, SkipRNN \cite{campos2017skip} extends classic RNN models by learning an additional controller network that learns to skip state updates. 
The input of this neuron is the state value of other neurons. So it can generate a binary value based on the sigmoid function value of its state. This model can significantly reduce the computational cost. 
However, while both RNNs and SNNs are used to deal with sequence analysis, they remain completely different. 
The main difference is that neurons in RNNs are mostly non-linear, continuous function approximators that operate on a common clock cycle, whereas the neurons in SNNs use asynchronous spikes that signal the occurrence of some characteristic event and temporally precise membrane potentials. When dealing with spiking training tasks, many neurons of an SNN may stay silent based on its mechanism, whereas all neurons of an RNN will be activated. 
Consequently, in terms of inference efficiency, RNNs are outmatched by SNNs for spike train classification. 
We illustrate this key difference in Figure~\ref{fig:intro2}.

==> sec_checklist.tex <==
\newpage

\section*{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\noindent{This paper:}

\textbullet  \  Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA). Answer: \textcolor{blue}{[yes]}

\textbullet  \ Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no). Answer: \textcolor{blue}{[yes]}

\textbullet  \ Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no). Answer: \textcolor{blue}{[yes]}

\vspace{8pt}

\noindent{Does this paper make theoretical contributions? (yes/no). Answer: \textcolor{blue}{[No]}}

\noindent{If yes, please complete the list below.}

\textbullet  \ All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

\textbullet  \ All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

\textbullet  \ Proofs of all novel claims are included. (yes/partial/no)

\textbullet  \ Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

\textbullet  \ Appropriate citations to theoretical tools used are given. (yes/partial/no)

\textbullet  \ All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

\textbullet  \ All experimental code used to eliminate or disprove claims is included. (yes/no/NA)

\vspace{8pt}

\noindent{Does this paper rely on one or more datasets? (yes/no)}. Answer: \textcolor{blue}{[Yes]}

\noindent{If yes, please complete the list below.}

\textbullet  \ A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA). Answer: \textcolor{blue}{[yes]}

\textbullet  \ All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA). Answer: \textcolor{blue}{[yes]}

\textbullet  \ All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA). Answer: \textcolor{blue}{[yes]}

\textbullet  \ All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA). Answer: \textcolor{blue}{[yes]}

\textbullet  \ All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA). Answer: \textcolor{blue}{[yes]}

\textbullet  \ All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA). Answer: \textcolor{blue}{[NA]}

\vspace{8pt}

\noindent{Does this paper include computational experiments? (yes/no)}. Answer: \textcolor{blue}{[yes]}

\noindent{If yes, please complete the list below.}

\textbullet  \ Any code required for pre-processing data is included in the appendix. (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ This paper states the number of algorithm runs used to compute each reported result. (yes/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no). Answer: \textcolor{blue}{[Yes]}

This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA). Answer: \textcolor{blue}{[Yes]}

\textbullet  \ This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA). Answer: \textcolor{blue}{[Yes]}

==> tab_ablation.tex <==
\begin{table*}[t]
    \centering
    \caption{Ablation studies on holding out tasks of UniBrain on ADHD dataset}
    \label{tab: ablation ADHD}
    \vspace{-5pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule

    \multicolumn{1}{c}{\multirow{2}{*}{Methods}} & 
    \multicolumn{2}{c}{Extraction} &
    \multicolumn{2}{c}{Registration} &
    \multicolumn{2}{c}{Segmentation} &
    \multicolumn{2}{c}{Parcellation} &
    \multicolumn{2}{c}{Classification}
    
    \\

    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
    \cmidrule(lr){10-11}

    \multicolumn{1}{c}{} &
    Dice $\uparrow$ &
    Jaccard $\uparrow$ &
    MI $\uparrow$ &
    CC $\uparrow$ &
    Dice $\uparrow$ &
    Jaccard $\uparrow$ &
    Dice $\uparrow$ &
    Jaccard $\uparrow$ &
    ACC $\uparrow$ &
    AUC-ROC $\uparrow$

    \\
    
    \midrule

    UniBrain w/o Ext &
    
    0.140 $\pm$ 0.009 &
    0.075 $\pm$ 0.005 &
    0.593 $\pm$ 0.015 &
    0.846 $\pm$ 0.029 &
    0.260 $\pm$ 0.039 &
    0.157 $\pm$ 0.028 &
    0.196 $\pm$ 0.096 &
    0.120 $\pm$ 0.063 &
    0.525 $\pm$ 0.038 &
    0.591 $\pm$ 0.023 

    \\

    UniBrain w/o Reg &

    0.968 $\pm$ 0.005 &
    0.938 $\pm$ 0.009 &
    0.362 $\pm$ 0.040 &
    0.706 $\pm$ 0.043 &
    0.286 $\pm$ 0.034 &
    0.175 $\pm$ 0.025 &
    0.140 $\pm$ 0.075 &
    0.086 $\pm$ 0.050 &
    0.571 $\pm$ 0.054 &
    0.605 $\pm$ 0.045 

    \\

    UniBrain w/o Seg &
    
    0.968 $\pm$ 0.004 &
    0.938 $\pm$ 0.007 &
    0.650 $\pm$ 0.005 &
    0.956 $\pm$ 0.008 &
    0.044 $\pm$ 0.028 &
    0.023 $\pm$ 0.015 &
    0.706 $\pm$ 0.019 &
    0.555 $\pm$ 0.021 &
    0.650 $\pm$ 0.032 &
    0.696 $\pm$ 0.029 

    \\

    UniBrain w/o Parc &
    
    0.969 $\pm$ 0.004 &
    0.941 $\pm$ 0.007 &
    0.651 $\pm$ 0.007 &
    0.955 $\pm$ 0.006 &
    0.514 $\pm$ 0.011 &
    0.380 $\pm$ 0.010 &
    0.140 $\pm$ 0.088 &
    0.086 $\pm$ 0.058 &
    0.569 $\pm$ 0.066 &
    0.590 $\pm$ 0.031 

    \\

    UniBrain w/o BN &
    
    0.968 $\pm$ 0.003 &
    0.939 $\pm$ 0.006 &
    0.648 $\pm$ 0.007 &
    0.956 $\pm$ 0.009 &
    0.518 $\pm$ 0.015 &
    0.375 $\pm$ 0.015 &
    0.706 $\pm$ 0.021 &
    0.555 $\pm$ 0.023 &
    0.583 $\pm$ 0.061 &
    0.631 $\pm$ 0.028 

    \\

    UniBrain w/o CLS &
    
    0.967 $\pm$ 0.004 &
    0.937 $\pm$ 0.007 &
    0.651 $\pm$ 0.009 &
    0.956 $\pm$ 0.008 &
    0.512 $\pm$ 0.012 &
    0.367 $\pm$ 0.012 &
    0.706 $\pm$ 0.020 &
    0.555 $\pm$ 0.022 &
    0.478 $\pm$ 0.000 &
    0.500 $\pm$ 0.000 

    \\
    
    \midrule
    \textbf{UniBrain} &

    \textbf{0.970 $\pm$ 0.003} &
    \textbf{0.942 $\pm$ 0.006} &
    \textbf{0.652 $\pm$ 0.008} &
    \textbf{0.957 $\pm$ 0.008} &
    \textbf{0.520 $\pm$ 0.013} &
    \textbf{0.381 $\pm$ 0.013} &
    \textbf{0.708 $\pm$ 0.019} &
    \textbf{0.557 $\pm$ 0.022} &
    \textbf{0.652 $\pm$ 0.027} &
    \textbf{0.712 $\pm$ 0.030} 

    \\

    \bottomrule    
    \end{tabular}}
    \vspace{-5pt}
\end{table*}



==> tab_datasets.tex <==
\begin{table}[h]
    \centering
    \vspace{-8pt}
    \caption{Summary of datasets}
    \label{tab:dataset}
    \vspace{-8.5pt}
    \resizebox{0.88\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
     & \textbf{LPBA40}& \textbf{CC359 }& \textbf{IBSR}\\
    \midrule
    Raw size  & $256\times124\times256$ & $171\times256\times256$ & $256\times256\times128$\\
    Cropped size  & $96\times96\times96$ & $96\times96\times96$ & $96\times96\times96$\\
    Training & 30  & 298 & -\\
    Validation & 5  & 30 & -\\
    Test & 4  & 30 & 18\\
    \bottomrule
    \end{tabular}}
    \vspace{-6pt}
\end{table}


==> tab_main_res_v2.tex <==

\begin{table*}[t]
    \centering
    \caption{Results for brain extraction (Ext), registration (Reg) and segmentation (Seg) in different datasets. The results are reported as performance(mean $\pm$ std ) of extraction, registration and segmentation of each compared method.
    “$\uparrow$” point out “the larger the better”. 
    The best results are highlighted in bold.}
    \label{tab:main res}
    \vspace{-10pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lccccccccccc}
    \toprule
    \multicolumn{3}{c}{\multirow{2}{*}{Methods}}                & \multicolumn{9}{c}{Datasets}   \\                                                    
    \cmidrule(lr){4-12}
    
    \multicolumn{3}{c}{}                                        & \multicolumn{3}{c}{LPBA40} & \multicolumn{3}{c}{CC359} & \multicolumn{3}{c}{IBSR}\\
    
    \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
    
    \multirow{2}{*}{Ext} & \multirow{2}{*}{Reg} & \multirow{2}{*}{Seg} & Ext  & Reg & Seg & Ext & Reg  & Seg & Ext & Reg & Seg \\   
                                    &     &    &
 Dice$_{\mathrm{ext}}$  $\uparrow$        & MI  $\uparrow$   &  Dice$_{\mathrm{seg}}$ $\uparrow$ 
 & Dice$_{\mathrm{ext}}$ $\uparrow$       & MI  $\uparrow$  & Dice$_{\mathrm{seg}}$ $\uparrow$         & Dice$_{\mathrm{ext}}$ $\uparrow$       & MI  $\uparrow$    & Dice$_{\mathrm{seg}}$ $\uparrow$  \\

     \midrule

    BET \cite{smith2002fast} & FLIRT \cite{jenkinson2001global} & DW~\cite{jaderberg2015spatial} & 0.935  $\pm$   0.028 & 0.627  $\pm$  0.010 & 0.613  $\pm$  0.025  & 0.811  $\pm$ 0.087 &
 0.481  $\pm$ 0.024 &
 0.748  $\pm$ 0.062 &
 0.911  $\pm$ 0.038 &
 0.521  $\pm$ 0.022 &
 0.800  $\pm$ 0.010
\\

    3dSS \cite{cox1996afni} & FLIRT \cite{jenkinson2001global} & DW~\cite{jaderberg2015spatial} & 0.902  $\pm$  0.032 & 0.627  $\pm$ 0.010 & 0.601  $\pm$ 0.017 & 0.849  $\pm$ 0.037 &
 0.500  $\pm$ 0.014 &
 0.791  $\pm$ 0.034 &
   0.869  $\pm$ 0.039 &
0.508  $\pm$ 0.023  &
0.788  $\pm$ 0.021
\\

    BSE \cite{shattuck2002brainsuite} & FLIRT \cite{jenkinson2001global} &DW~\cite{jaderberg2015spatial} &0.938  $\pm$ 0.022
& 0.668  $\pm$ 0.010 &
0.620  $\pm$ 0.008  & 0.846  $\pm$ 0.112 &
0.518  $\pm$ 0.035 &
0.804  $\pm$ 0.019 &
 0.873  $\pm$ 0.064 &
0.521  $\pm$ 0.026 &
0.799  $\pm$ 0.015
 \\

    \midrule

    BET \cite{smith2002fast} & ANTs \cite{avants2009advanced} & DW~\cite{jaderberg2015spatial} & 0.935  $\pm$ 0.028 & 0.630  $\pm$ 0.013 &
0.625  $\pm$ 0.010  & 0.811  $\pm$ 0.087 &
0.476  $\pm$ 0.027 &
0.744  $\pm$ 0.062 &
 0.911  $\pm$ 0.038 &
0.524  $\pm$ 0.022 &
0.792  $\pm$ 0.018

 \\

    3dSS \cite{cox1996afni} & ANTs \cite{avants2009advanced} & DW~\cite{jaderberg2015spatial} & 0.902  $\pm$ 0.032 &
0.632  $\pm$ 0.011 &
0.524  $\pm$ 0.133  & 0.849  $\pm$ 0.037 &
0.498  $\pm$ 0.016 &
0.758  $\pm$ 0.041 &
 0.869  $\pm$ 0.039 &
0.508  $\pm$ 0.026 &
0.762  $\pm$ 0.030\\

    BSE \cite{shattuck2002brainsuite} & ANTs \cite{avants2009advanced} &DW~\cite{jaderberg2015spatial} & 0.938  $\pm$ 0.022 &
0.671  $\pm$ 0.008 &
0.614  $\pm$ 0.023  & 0.846  $\pm$ 0.112 &
0.524  $\pm$ 0.035 &
0.807  $\pm$ 0.012 &
 0.873  $\pm$ 0.064 &
0.522  $\pm$ 0.027 &
0.787  $\pm$ 0.016\\
    \midrule

        BET \cite{smith2002fast} & VM \cite{balakrishnan2018unsupervised} & DW~\cite{jaderberg2015spatial} & 0.935  $\pm$ 0.028 &
0.627 $\pm$ 0.016 &
0.607 $\pm$ 0.019  & 0.811  $\pm$ 0.087 &
0.465 $\pm$ 0.034 &
0.804 $\pm$ 0.015 &
 0.911  $\pm$ 0.038 &
0.525 $\pm$ 0.023 &
0.795 $\pm$ 0.013 \\

    3dSS \cite{cox1996afni} & VM \cite{balakrishnan2018unsupervised} & DW~\cite{jaderberg2015spatial} &0.902  $\pm$ 0.032 &
0.623 $\pm$ 0.009 &
0.590 $\pm$ 0.009  & 0.849  $\pm$ 0.037 &
0.496 $\pm$ 0.018 &
0.814 $\pm$ 0.007 &
 0.869  $\pm$ 0.039 &
0.509 $\pm$ 0.027 &
0.789 $\pm$ 0.017\\

    BSE \cite{shattuck2002brainsuite} & VM \cite{balakrishnan2018unsupervised} &DW~\cite{jaderberg2015spatial} & 0.938  $\pm$ 0.022 &
0.670 $\pm$ 0.003 &
0.616 $\pm$ 0.010  & 0.846  $\pm$ 0.112 &
0.515 $\pm$ 0.041 &
0.805 $\pm$ 0.016 &
 0.873  $\pm$ 0.064 &
0.524 $\pm$ 0.028 &
0.795 $\pm$ 0.013\\
    \midrule

    BET \cite{smith2002fast} & CRN \cite{zhao2019recursive} & DW~\cite{jaderberg2015spatial} & 0.935  $\pm$ 0.028 &
0.633 $\pm$ 0.017 &
0.618 $\pm$ 0.022  & 0.811  $\pm$ 0.087 &
0.467 $\pm$ 0.034 &
0.806 $\pm$ 0.015 &
 0.911  $\pm$ 0.038 &
0.527 $\pm$ 0.023 &
0.800 $\pm$ 0.011\\

    3dSS \cite{cox1996afni} & CRN \cite{zhao2019recursive} & DW~\cite{jaderberg2015spatial} & 0.902  $\pm$ 0.032 &
0.630 $\pm$ 0.012 &
0.610 $\pm$ 0.013  & 0.849  $\pm$ 0.037 &
0.498 $\pm$ 0.017 &
0.817 $\pm$ 0.007 &
 0.869  $\pm$ 0.039 &
0.513 $\pm$ 0.028 &
0.794 $\pm$ 0.014\\

    BSE \cite{shattuck2002brainsuite} & CRN \cite{zhao2019recursive} &DW~\cite{jaderberg2015spatial} & 0.938  $\pm$ 0.022 &
0.674 $\pm$ 0.006 &
0.626 $\pm$ 0.010  & 0.846  $\pm$ 0.112 &
0.518 $\pm$ 0.040 &
0.809 $\pm$ 0.017 &
 0.873  $\pm$ 0.064 &
0.527 $\pm$ 0.028 &
0.796 $\pm$ 0.013\\
    \midrule

        BET \cite{smith2002fast} & \multicolumn{2}{c}{DeepAtlas \cite{xu2019deepatlas}} & 0.935  $\pm$ 0.028 & 0.627 $\pm$ 0.016 & 0.645 $\pm$ 0.009  & 0.811  $\pm$ 0.087 &
0.467 $\pm$ 0.033 &
0.814 $\pm$ 0.017 &
 0.911  $\pm$ 0.038 &
0.524 $\pm$ 0.024 &
0.811 $\pm$ 0.011 \\

    3dSS \cite{cox1996afni} & \multicolumn{2}{c}{DeepAtlas \cite{xu2019deepatlas}} & 0.902  $\pm$ 0.032 & 0.625 $\pm$ 0.013 & 0.640 $\pm$ 0.010  & 0.849  $\pm$ 0.037 &
0.498 $\pm$ 0.018 &
0.828 $\pm$ 0.007 &
 0.869  $\pm$ 0.039 &
0.509 $\pm$ 0.027 &
0.808 $\pm$ 0.013\\

    BSE \cite{shattuck2002brainsuite} & \multicolumn{2}{c}{DeepAtlas \cite{xu2019deepatlas}} & 0.938  $\pm$ 0.022 &
0.667 $\pm$ 0.006 &
0.648 $\pm$ 0.009  & 0.846  $\pm$ 0.112 &
0.518 $\pm$ 0.041 &
0.817 $\pm$ 0.017 &
 0.873  $\pm$ 0.064 &
0.525 $\pm$ 0.029 &
0.807 $\pm$ 0.014\\
    \midrule

    \multicolumn{2}{c}{ERNet \cite{su2022ernet}} & DW~\cite{jaderberg2015spatial} & 0.942 $\pm$ 0.010 &
0.675 $\pm$ 0.004 &
0.620 $\pm$ 0.012  & 0.935 $\pm$ 0.006 &
0.573 $\pm$ 0.007 &
0.818 $\pm$ 0.007 &
 0.915 $\pm$ 0.019 &
0.544 $\pm$ 0.029 &
0.799 $\pm$ 0.012\\
    \midrule
    \multicolumn{3}{c}{\textbf{JERS (ours)}} &
   \textbf{ 0.944 $\pm$ 0.008} &
\textbf{0.679 $\pm$ 0.005} &
\textbf{0.651 $\pm$ 0.011}  & \textbf{0.937 $\pm$ 0.005} &
\textbf{0.574 $\pm$ 0.006} &
\textbf{0.840 $\pm$ 0.010} &
 \textbf{0.917 $\pm$ 0.019} &
\textbf{0.550 $\pm$ 0.025} &
\textbf{0.832 $\pm$ 0.010}
\\
    
    \bottomrule    
    \end{tabular}}
    \vspace{-10pt}
\end{table*}



==> tab_notation.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Basic Notation.}
%     \label{tab: Notation}
    
%     \begin{tabular}{ll}
%     \toprule
%     Notation& Description\\
%     \midrule
%     $W$, $H$, $D$& Spatial dimension of images (width, height and depth)\\
%     $n$& Number of stages\\ 
%     $\mathbf{I}_{m}$& Moving source images\\
%     $\mathbf{I}_{f}$& Fixed target images\\
%     $\mathbf{I}_{w}^{(k)}$& Intermediate warped registered images at stage $k$\\
%     $\mathbf{I}_{w}^{(n)}$& Final warped registered images at stage $n$\\
%     $\phi$& Deformation field - transformation between images\\
%     $\phi_L^{(k)}$& Local deformation field between $\mathbf{I}_{w}^{(k-1)}$ and $\mathbf{I}_{f}$ at stage $k$\\ 
%     $\phi_G^{(k)}$& Global deformation field between $\mathbf{I}_{m}$ and $\mathbf{I}_{f}$ at stage $k$\\ 
%     $\mathcal{T}$& Warping operation - resamples the image by given $\phi$ \\
%     \midrule
%      & Where $k=[1, \ldots, n]$\\
%     \bottomrule
%     \end{tabular}
% \end{table}
\newpage
\begin{table*}[ht]
    \centering
    \caption{Basic Notation.}
    \label{tab: Notation}
    \vspace{-0pt}
    \begin{tabularx}{1.0\linewidth}{lX}
    \toprule
    Notation& Description\\
    \midrule

    $W$, $H$, $D$& 
    width, height and depth dimensions of the 3D images\\
    
    % $W$, $H$, $D$& Spatial dimension of the image (width, height and depth).\\
    %$\mathcal{D} = \{\{\mathbf{S}_\text{1}, \cdots, \mathbf{S}_\text{Z} \},\mathbf{T}\}$ & the given unlabeled dataset, $\mathbf{S}_{i}$ denotes the $i$-th source image in the dataset. \\
    
    $\mathbf{S}_i$ &
    source image (\ie raw MRI scan), $\mathbf{S}_{i} \in \mathbb{R}^{W \times H \times D}$ \\

    $\mathbf{M}_i$ &
    ground truth brain extraction mask of $\mathbf{S}_i$, $\mathbf{M}_i \in \{0,1\}^{W \times H \times D}$\\

    $y_i$ &
    ground truth classification label of $\mathbf{S}_i$, $y_i \in \mathcal{Y}$\\

    $\mathcal{Y}$ &
    classification label space (\eg $\{0, 1\}$ for binary classification)\\

    $\mathcal{D} = \{(\mathbf{S}_i,\mathbf{M}_i,y_i)\}_{i=1}^{Z}$ &
    dataset contains $Z$ source images, each paired with a brain extraction mask $\mathbf{M}_i$ and classification label $y_i$ \\

    $\mathbf{T}$ &
    target image, $\mathbf{T} \in \mathbb{R}^{W \times H \times D}$\\

    $\mathbf{B}$ &
    segmentation mask of $\mathbf{T}$, $\mathbf{B} \in \{0, 1\}^{C \times W \times H \times D}$\\

    $\mathbf{P}$ &
    parcellation mask of $\mathbf{T}$, $\mathbf{P} \in \{0, 1\}^{K \times W \times H \times D}$\\

    
    $C$ &
    number of segmentation labels (\ie the number of labeled brain tissue types)\\

    $K$ &
    number of labeled brain regions (\ie the number of ROIs)\\


    \midrule
    % $\hat{\mathbf{M}}_i$ &
    % binary tensor of identical dimensions to the source image $\mathbf{S}_i$, represents cerebral tissues in $\mathbf{S}$ with a value of 1 and non-cerebral tissues with 0\\

     $\hat{\mathbf{M}}$ &
    predicted brain extraction mask, $\hat{\mathbf{M}} \in \{0, 1\}^{W \times H \times D}$\\
    % \midrule
    
    $\hat{y}$&
    predicted classification label, $\hat{y} \in \mathcal{Y}$\\

    $\mathbf{E}$ &
    extracted image, obtained by $\mathbf{E} = \mathbf{S} \circ \hat{\mathbf{M}}$, $\mathbf{E}  \in \mathbb{R}^{W \times H \times D}$\\

    $\mathbf{a}$ &
    vector of the affine transformation, $\mathbf{a} \in \mathbb{R}^{12} $ \\  
    
    $\mathbf{A}$&
    matrix of an 3D affine transformation, $\mathbf{A} \in \mathbb{R}^{4 \times 4} $ \\

    $\mathcal{T}(\cdot, \cdot)$&
    affine transformation operator\\
    
    $\mathbf{W}$ &
    warped image, obtained by $\mathbf{W} = \mathcal{T}\left(\mathbf{E},\mathbf{A}\right)$\\

    $\mathbf{R}$&
    source segmentation mask, $\mathbf{R} \in \{0,1\}^{C \times W \times H \times D}$\\

    $\mathbf{V}$&
    warped segmentation mask, $\mathbf{V} \in \{0,1\}^{C \times W \times H \times D}$\\

    $\mathbf{U}$&
    warped parcellation mask, $\mathbf{U} \in \{0,1\}^{K \times W \times H \times D}$\\

    $\tilde{\mathbf{S}}$&
    source images expanded from $\mathbf{S}$ for ROI extraction, $\tilde{\mathbf{S}} \in \mathbb{R}^{K \times W \times H \times D}$\\

    $\mathbf{F}$&
    ROI extracted image (\ie parcellated image), obtained by $\mathbf{F} = \tilde{\mathbf{S}} \circ \mathbf{U}$, $\mathbf{F} \in \mathbb{R}^{K \times W \times H \times D}$\\
    
    $\mathbf{H}$&
    matrix of ROI feature (\ie node feature), $\mathbf{H} \in \mathbb{R}^{K \times N}$\\

    $N$&
    feature vector length of $\mathbf{H}$\\

    $\mathbf{C}$&
    adjacency matrix, measures brain network connectivity, $\mathbf{C} \in \mathbb{R}^{K \times K}$\\


     %\midrule
    $\mathcal{V}$&
    set of nodes (\ie ROIs), $\mathcal{V}=\{v_j\}_{j=1}^{K}$\\
    % \midrule
    
    $G$&
    brain network, $G = (\mathcal{V},\mathbf{C},\mathbf{H})$\\
    \midrule
    $f_{\theta}(\cdot)$&
    extraction function, $f_{\theta}: \mathbb{R}^{W \times H \times D} \rightarrow \mathbb{R}^{W \times H \times D} ; \mathbf{S} \mapsto \hat{\mathbf{M}}$\\

    $g_{\phi}(\cdot, \cdot)$&
    registration function, $g_{\phi}: \mathbb{R}^{W \times H \times D}\times \mathbb{R}^{W \times H \times D} \rightarrow \mathbb{R}^{12} ; (\mathbf{E},\mathbf{T}) \mapsto \mathbf{A}$\\

    $h_{\psi}(\cdot)$&
    segmentation function $h_{\psi}: \mathbb{R}^{W \times H \times D} \rightarrow \mathbb{R}^{C \times W \times H \times D} ; \mathbf{S} \mapsto \mathbf{R} $\\

    $n_{\xi}(\cdot)$&
    brain network generation function, $n_{\xi}: \mathbb{R}^{K \times W \times H \times D} \rightarrow \mathbb{R}^{K \times N} ; \mathbf{F} \mapsto \mathbf{H} $\\

    $c_{\eta}(\cdot,\cdot)$&
    classification function $c_{\eta}: (\mathbb{R}^{K \times K}, \mathbb{R}^{K \times N}) \rightarrow \mathcal{Y} ; (\mathbf{C},\mathbf{H}) \mapsto \hat{y}$\\

    $\mathcal{P^*}$&
    optimal parameter set, $\mathcal{P^*} = \{\theta^*, \phi^*, \psi^*, \xi^*, \eta^*\}$\\

    $\mathcal{L}_{cls}(\cdot, \cdot)$ &
    classification loss term, \ie cross-entropy loss\\

    $\mathcal{L}_{ext}(\cdot, \cdot)$ &
    extraction loss term, \ie cross-entropy loss\\

    $\mathcal{L}_{sim}(\cdot, \cdot)$ &
    image dissimilarity loss term, \ie negative cross-correlation\\

    $\mathcal{L}_{seg}(\cdot, \cdot)$ &
    segmentation loss term, \ie cross-entropy loss\\
    
    
    % \\\\
    
    % $M$, $N$& 
    % the number of extraction stages, the number of registration stages. \\
    
    % $\mathbf{S}_{i}$ & the source image (to be extracted and registered with the target image), $\mathbf{S}_{i} \in \mathbb{R}^{W \times H \times D} $.  \\
    % $\mathbf{T}$ & the target image (template brain), $\mathbf{T} \in \mathbb{R}^{W \times H \times D}$.\\
    % $\mathcal{D} = \{\{\mathbf{S}_{i}\},\mathbf{T}\}_{i=1}^{Z}$ & the unlabeled dataset consists of $Z$ source images and one target image (no extraction and registration labels).\\
    % $\mathbf{E}_{i}$ & the extracted image (extracted brain region from the source image $\mathbf{S}_{i}$), $\mathbf{E} \in \mathbb{R}^{W \times H \times D}$.\\
    % $\mathbf{E}_{i}^{j}$ & the extracted image at extraction stage $j$, where $j \in [1 : M]$.\\
    % $\mathbf{W}_{i}$ & the warped image (image that has been registered to the target image $\mathbf{T}$), $\mathbf{W} \in \mathbb{R}^{W \times H \times D}$.\\
    % $\mathbf{W}_{i}^{k}$ & the warped image at registration stage $k$, where $k \in [1 : N]$.\\
    % $\mathbf{M}_{i}$&  the binary brain mask (to extracted the brain region from the source image $\mathbf{S}_{i}$), $\mathbf{M}_{i} \in \{0,1\}^{W \times H \times D}$.\\
    % $\mathbf{M}_{i}^{j}$& the binary brain mask at extraction stage $j$, where $j \in [1 : M]$.\\
    % $\mathbf{a}_{i}$& the vector of the affine transformation parameters, $\mathbf{a}_{i} \in \mathbb{R}^{12}$.\\
    % $\mathbf{A}_{i}$& the matrix of the affine transformation, $\mathbf{A}_{i} \in \mathbb{R}^{4 \times 4}$.\\
    % ${\mathbf{A}_\text{i}}_{i}^{k}$ & the matrix of the current affine transformation between $\mathbf{W}_{i}^{k-1}$ and $\mathbf{T}$ at registration stage $k$, where $k \in [1 : N]$.\\
    % ${\mathbf{A}_\text{c}}_{i}^{k}$ & the matrix of the combined affine transformation between $\mathbf{E}_{i}$ and $\mathbf{T}$ at registration stage $k$, where $k \in [1 : N]$.\\
    % $\mathcal{T}(\cdot, \cdot)$& the affine warping operation. \\
    
    
    
    
    
    
    
    
    
    % $\mathbf{I}_\text{s}$& The source image (to be extracted and registered with the target image).\\
    % \vspace{1pt}
    % $\mathbf{I}_\text{t}$& The target image (template brain).\\
    % \vspace{1pt}
    % $\mathbf{I}_\text{e}^{(j)}$& The extracted image at stage $j$.\\
    % \vspace{1pt}
    % $\mathbf{I}_\text{w}^{(k)}$& The warped image at stage $k$.\\
    % $\mathbf{M}$&  Binary brain mask.\\
    % $\mathbf{M}^{(j)}$& Current brain mask of $\mathbf{I}_\text{e}^{(j-1)}$ at stage $j$.\\
    % $\mathbf{a}$& Affine transformation parameters.\\
    % $\mathbf{A}$& Affine transformation matrix.\\
    % $\mathbf{A}_\text{i}^{(k)}$& Current affine transformation between $\mathbf{I}_\text{w}^{(k-1)}$ and $\mathbf{I}_\text{t}$ at stage $k$.\\
    % $\mathbf{A}_\text{c}^{(k)}$& Combined affine transformation between $\mathbf{I}_\text{s}$ and $\mathbf{I}_\text{t}$ at stage $k$.\\

    % $\mathcal{T}$& Affine warping operation. \\
    
    % \midrule
    %  & where $j=[1, \ldots, m]$ and $k=[1, \ldots, n]$  \\
    \bottomrule
    \end{tabularx}
    \vspace{-0pt}
\end{table*}

==> tab_res_ABIDE.tex <==

\begin{table*}[t]
    \centering
    \caption{Results on ABIDE dataset. The results are reported as (mean $\pm$ std ) of each task for each compared method.
    “$+$” indicates combining different baselines for the corresponding tasks.}
    \label{tab:res ABIDE}
    \vspace{-7pt}
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{ccccccccccc}
    \toprule
    % \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Methods}}              & 
    \multicolumn{2}{c}{Extraction}             &
    \multicolumn{2}{c}{Registration}    &
    \multicolumn{2}{c}{Segmentation}    &
    \multicolumn{2}{c}{Parcellation}    &
    \multicolumn{2}{c}{Classification}
    
    \\   
    
    % \cmidrule(lr){1-6}
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
    \cmidrule(lr){10-11}
    % \hline
    
    
    
    
    
    
    % {Ext}                                        & 
    % {Reg}             &
    % {Seg}             &
    % {Parc}        &
    % {NG}        &
    % {Cls}         &
    {} &
    
    {Dice $\uparrow$} & 
    {Jaccard $\uparrow$} & 
    
    {MI $\uparrow$} &
    {CC $\uparrow$} &

    {Dice $\uparrow$} &
    {Jaccard $\uparrow$} &

    {Dice $\uparrow$} &
    {Jaccard $\uparrow$} &

    {ACC $\uparrow$} &
    {AUC-ROC $\uparrow$} 
    

    \\
    
    \midrule
    % \hline
    
    
    BET +
    FLIRT + 
    DW +
    KNN +
    GCN &
    
    0.786 $\pm$ 0.173 &
    0.673 $\pm$ 0.180 &
    0.575 $\pm$ 0.029 &
    0.890 $\pm$ 0.036 &
    0.411 $\pm$ 0.074 &
    0.279 $\pm$ 0.061 &
    0.525 $\pm$ 0.183 &
    0.388 $\pm$ 0.152 &
    0.521 $\pm$ 0.013 &
    0.567 $\pm$ 0.004 

    \\   

    % \cmidrule(lr){1-6}
    % \hline
    
    Synth +
    FLIRT +
    DW +
    KNN +
    GCN  &
    
    0.909 $\pm$ 0.026 &
    0.835 $\pm$ 0.042 &
    0.613 $\pm$ 0.026 &
    0.938 $\pm$ 0.010 &
    0.474 $\pm$ 0.026 &
    0.331 $\pm$ 0.023 &
    0.670 $\pm$ 0.043 &
    0.516 $\pm$ 0.043 &
    0.551 $\pm$ 0.046 &
    0.610 $\pm$ 0.007 

    \\

    % \cmidrule(lr){1-6}
    % \hline
    

    BET +
    VM +
    DW + 
    KNN +
    GCN  &
    
    0.786 $\pm$ 0.173 &
    0.673 $\pm$ 0.180 &
    0.577 $\pm$ 0.026 &
    0.897 $\pm$ 0.039 &
    0.385 $\pm$ 0.072 &
    0.257 $\pm$ 0.059 &
    0.466 $\pm$ 0.182 &
    0.334 $\pm$ 0.148 &
    0.524 $\pm$ 0.018 &
    0.574 $\pm$ 0.005 
    
    \\

    % \cmidrule(lr){1-6}
    % \hline
    
    Synth +
    VM +
    DW +
    KNN +
    GCN   &
    
    0.909 $\pm$ 0.026 &
    0.835 $\pm$ 0.042 &
    0.611 $\pm$ 0.023 &
    0.948 $\pm$ 0.010 &
    0.454 $\pm$ 0.026 &
    0.314 $\pm$ 0.022 &
    0.642 $\pm$ 0.046 &
    0.487 $\pm$ 0.045 &
    0.543 $\pm$ 0.021 &
    0.552 $\pm$ 0.005 

    \\
    
    % \cmidrule(lr){1-6}
    % \hline
    
    
    BET +
    ABN +
    DW + 
    KNN +
    GCN   &
    
    0.786 $\pm$ 0.173 &
    0.673 $\pm$ 0.180 &
    0.577 $\pm$ 0.024 &
    0.900 $\pm$ 0.037 &
    0.385 $\pm$ 0.077 &
    0.258 $\pm$ 0.063 &
    0.486 $\pm$ 0.188 &
    0.353 $\pm$ 0.155 &
    0.553 $\pm$ 0.012 &
    0.568 $\pm$ 0.002 
    
    \\

    % \cmidrule(lr){1-6}
    % \hline
    
    Synth +
    ABN +
    DW +
    KNN +
    GCN   &
    
    0.909 $\pm$ 0.026 &
    0.835 $\pm$ 0.042 &
    0.612 $\pm$ 0.023 &
    0.950 $\pm$ 0.010 &
    0.457 $\pm$ 0.026 &
    0.317 $\pm$ 0.023 &
    0.661 $\pm$ 0.048 &
    0.507 $\pm$ 0.047 &
    0.565 $\pm$ 0.024 &
    0.579 $\pm$ 0.005 

    \\

    % \cmidrule(lr){1-6}
    % \hline
    

    ERNet + 
    DW + 
    KNN +
    GCN   &
    
    0.927 $\pm$ 0.019 &
    0.866 $\pm$ 0.032 &
    0.627 $\pm$ 0.018 &
    0.958 $\pm$ 0.009 &
    0.483 $\pm$ 0.022 &
    0.337 $\pm$ 0.019 &
    0.652 $\pm$ 0.053 &
    0.497 $\pm$ 0.054 &
    0.554 $\pm$ 0.019 &
    0.590 $\pm$ 0.008 

    \\

    % \cmidrule(lr){1-6}
    % \hline
    

    BET + 
    DeepAtlas + 
    DW + 
    KNN +
    GCN   &
    
    0.786 $\pm$ 0.173 &
    0.673 $\pm$ 0.180 &
    0.576 $\pm$ 0.024 &
    0.898 $\pm$ 0.038 &
    0.394 $\pm$ 0.077 &
    0.268 $\pm$ 0.064 &
    0.469 $\pm$ 0.182 &
    0.337 $\pm$ 0.148 &
    0.524 $\pm$ 0.015 &
    0.562 $\pm$ 0.015 
    
    \\

    % \cmidrule(lr){1-6}
    % \hline
    
    Synth +
    DeepAtlas +
    DW +
    KNN +
    GCN &
    
    0.909 $\pm$ 0.026 &
    0.835 $\pm$ 0.042 &
    0.613 $\pm$ 0.023 &
    0.949 $\pm$ 0.010 &
    0.471 $\pm$ 0.028 &
    0.334 $\pm$ 0.025 &
    0.647 $\pm$ 0.051 &
    0.492 $\pm$ 0.050 &
    0.557 $\pm$ 0.032 &
    0.572 $\pm$ 0.004 

    \\

    % \cmidrule(lr){1-6}
    % \hline
    

    JERS +
    DW +
    KNN  +
    GCN   &
    
    0.929 $\pm$ 0.017 &
    0.869 $\pm$ 0.030 &
    0.628 $\pm$ 0.018 &
    0.959 $\pm$ 0.009 &
    0.508 $\pm$ 0.026 &
    0.364 $\pm$ 0.024 &
    0.655 $\pm$ 0.050 &
    0.501 $\pm$ 0.051 &
    0.551 $\pm$ 0.022 &
    0.591 $\pm$ 0.006 

    \\

    % \cmidrule(lr){1-6}
    % \hline
    
    JERS +
    DW +
    KNN +
    BGN   &
    
    0.929 $\pm$ 0.017 &
    0.869 $\pm$ 0.030 &
    0.628 $\pm$ 0.018 &
    0.959 $\pm$ 0.009 &
    0.508 $\pm$ 0.026 &
    0.364 $\pm$ 0.024 &
    0.655 $\pm$ 0.050 &
    0.501 $\pm$ 0.051 &
    0.529 $\pm$ 0.072 &
    0.534 $\pm$ 0.083 

    \\

    % \cmidrule(lr){1-6}
    % \hline
    
    JERS +
    DW +
    KNN +
    BNT   &
    
    0.929 $\pm$ 0.017 &
    0.869 $\pm$ 0.030 &
    0.628 $\pm$ 0.018 &
    0.959 $\pm$ 0.009 &
    0.508 $\pm$ 0.026 &
    0.364 $\pm$ 0.024 &
    0.655 $\pm$ 0.050 &
    0.501 $\pm$ 0.051 &
    0.571 $\pm$ 0.044 &
    0.605 $\pm$ 0.022 

    \\

    \midrule
    % \hline
    
    \textbf{UniBrain (ours)} &
    
    \textbf{0.970 $\pm$ 0.012} &
    \textbf{0.942 $\pm$ 0.021} &
    \textbf{0.641 $\pm$ 0.015} &
    \textbf{0.965 $\pm$ 0.007} &
    \textbf{0.515 $\pm$ 0.024} &
    \textbf{0.367 $\pm$ 0.022} &
    \textbf{0.692 $\pm$ 0.035} &
    \textbf{0.540 $\pm$ 0.037} &
    \textbf{0.648 $\pm$ 0.043} &
    \textbf{0.781 $\pm$ 0.029} 

    \\
    
    \bottomrule   
    % \hline
    
    \end{tabular}}
    \vspace{-7pt}
\end{table*}



==> tab_transformation.tex <==

\begin{table}[h]
    \centering
    \vspace{-0pt}
    \caption{Range of augmentation.}
    \label{tab:transformation}
    \vspace{-0pt}
    \resizebox{0.50\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    
    \multicolumn{3}{c}{Transformation} &
    \multicolumn{2}{c}{Perturbation}\\
    
    
    
    
    \cmidrule(lr){1-3}
    \cmidrule(lr){4-5}
    
        Translation  & Rotation & Scale & Feature & Edge         \\
        (Voxels)  & (Degree)  & (Times) & (Rate) & (Rate)    \\


    \midrule
    $\pm$ 2 & $\pm$ 2  & 0.98 $\sim$ 1.02 & 0.01 & 0.01\\
    
    

    
    \bottomrule
    \end{tabular}}
    \vspace{-0pt}
\end{table}
    

==> table1.tex <==
% Results Tables
\begin{table*}[t!]
\centering
\caption{Comparative results on N-MNIST dataset.}
\vspace{-5pt}
\label{tab:nmnist}
\begin{tabular}{cccc}
\hline
{Model} & {Percentage of awake state} & {Accuracy}&{Inference MFLOPs}\\
\hline
{SNN}    & 100\% $\pm$ 0.0\% & 88.92\% $\pm$ 0.76\% & 1.15 \\ {Fixed-skip SNN}    & 13.33\% $\pm$ 0.0\% & 38.43\% $\pm$ 4.13\% & 0.51 \\
{Random-skip SNN}    & 10.00\% $\pm$ 0.0\% & 37.16\% $\pm$ 3.41\% & 0.47 \\
{SkipRNN+SNN, $\lambda=10^{-3}$}    & 91.72\% $\pm$ 0.37\% & 89.86\% $\pm$ 0.16\% & 0.71 \\
{SkipRNN+SNN, $\lambda=10^{-1}$}    & 11.13\% $\pm$ 1.24\% & 81.24\% $\pm$ 1.02\% & 0.52 \\
\hline
{SkipSNN, $\lambda=10^{-3}$}    & 92.15\% $\pm$ 0.08\% & 94.47\% $\pm$ 0.12\% & 0.75 \\
{SkipSNN, $\lambda=10^{-1}$}    & 11.03\% $\pm$ 0.58\% & 86.65\% $\pm$ 0.27\% & 0.46 \\
\hline
\end{tabular}
\vspace{-5pt}
\end{table*}

==> table2.tex <==
% Results Tables
\begin{table*}[t!]
\centering
\caption{Comparative results on DVS-Gesture dataset.}
\vspace{-5pt}
\label{tab:dvs}
\begin{tabular}{cccc}
\hline
{Model} & {Percentage of awake state} & {Accuracy}&{Inference MFLOPs}\\
\hline
{SNN}    & 100\% $\pm$ 0.0\% & 86.12\% $\pm$ 0.25\% & 1232.5 \\ {Fixed-skip SNN}    & 13.33\% $\pm$ 0.0\% & 64.13\% $\pm$ 2.05\% & 147.4 \\
{Random-skip SNN}    & 10.00\% $\pm$ 0.0\% & 63.41\% $\pm$ 2.37\% & 112.5 \\
{SkipRNN+SNN, $\lambda=10^{-5}$}    & 92.41\% $\pm$ 0.42\% & 85.32\% $\pm$ 0.43\% & 1013.1 \\
{SkipRNN+SNN, $\lambda=10^{-4}$}    & 10.02\% $\pm$ 3.35\% & 78.50\% $\pm$ 0.43\% & 117.3 \\
\hline
{SkipSNN, $\lambda=10^{-6}$}    & 89.63\% $\pm$ 0.23\% & 86.82\% $\pm$ 0.13\% & 973.7 \\
{SkipSNN, $\lambda=10^{-4}$}    & 9.04\% $\pm$ 1.44\% & 80.24\% $\pm$ 0.18\% & 72.6 \\
\hline
\end{tabular}
\vspace{-5pt}
\end{table*}
